The DREAMS Project: Disentangling the Impact of Halo-to-Halo Variance and Baryonic Feedback on Milky Way Dark Matter Density Profiles

In this work, we utilize a new suite of Milky Way-mass halos from the DREAMS Project, simulated with Cold Dark Matter (CDM), to quantify the influence of baryon feedback and intrinsic halo-to-halo variance on dark matter density profiles. Our suite of 1024 halos varies over supernova and black hole feedback parameters from the IllustrisTNG model, as well as variations in two cosmological parameters. We find that, for the DREAMS parameter variations, Milky Way-mass dark matter density profiles in the IllustrisTNG model are largely insensitive to astrophysics and cosmology variations, with the dominant source of scatter instead arising from halo-to-halo variance. However, most of the (comparatively minor) feedback-driven variations come from the changes to supernova prescriptions. By comparing to dark matter-only simulations, we find that the strongest supernova wind energies are so effective at preventing galaxy formation that the halos are nearly entirely collisionless dark matter. Finally, regardless of physics variation, all the DREAMS halos are roughly consistent with a halo contracting adiabatically from the presence of baryons, unlike models that have bursty stellar feedback. This work represents a step toward assessing the uncertainty in Milky Way dark matter profiles, with direct implications for dark matter searches where systematic uncertainty in the density profile remains a major challenge.

==> tables/parameter_variations.tex <==
% \nolinenumbers
\begin{table*}
    \centering
    \begin{tabular}{p{0.1\linewidth}p{0.45\linewidth}p{0.2\linewidth}p{0.15\linewidth}}
        \toprule
         \textbf{Parameter} & \textbf{Brief Description} & \textbf{Fiducial TNG Value} & \textbf{Variations} \\\midrule
         $\bar{e}_w$ & SN Wind Energy & 3.6 & $[0.25$--4]$ \times3.6$ \\
         $\kappa_w$ & SN Wind Speed & 7.4 & $[0.5$--$2]\times7.4$\\
         $\epsilon_{f,\,\mathrm{high}}$ & AGN Feedback Strength & 0.1 & $[0.25$--$4]\times0.1$\\
         $\Omega_{\rm M}$ & Matter Density of Universe & 0.31 & $[0.274$--$0.354]$ \\
         $\sigma_8$ & Amplitude of Matter Clustering on 8 Mpc Scales & 0.8159 & $[0.780$--$0.888]$
         \\\bottomrule
    \end{tabular}
    \caption{{\bf Astrophysical and Cosmological Parameter Variations.}
    The astrophysical ($\bar{e}_w$, $\kappa_w$, $\epsilon_{f,\,\mathrm{high}}$) and cosmological ($\Omega_{\rm M}$, $\sigma_8$) parameters varied in the CDM DREAMS Milky Way-mass zoom-in simulations.
    We list the fiducial TNG value for each parameter, the variations used in these simulations (corresponding to a factor of $4$ for $\bar{e}_w$ and $\epsilon_{f,\,\mathrm{high}}$, a factor of $2$ for $\kappa_w$, and the two-standard-deviation uncertainty on \protect\citeauthor{Planck_2014}~\protect\citeyear{Planck_2014} for $\Omega_{\rm M}$ and $\sigma_8$).
    We sample the unique set of parameters for each simulation according to a \protect\cite{sobol} sequence.
    Finally, we note that $\bar{e}_w$, $\kappa_w$, and $\epsilon_{f,\,\mathrm{high}}$ are sampled in logarithmic space, whereas $\Omega_{\rm M}$ and $\sigma_8$ are sampled in linear space.
    Detailed justifications for these parameter ranges can be found in \protect\citetalias{Rose_2025}.
    }
    \label{tab:dreams_parameters}
\end{table*}
% \linenumbers
